MedTet: An Online Motion Model for 4D Heart Reconstruction

We present a novel approach to reconstruction of 3D cardiac motion from sparse intraoperative data. While existing methods can accurately reconstruct 3D organ geometries from full 3D volumetric imaging, they cannot be used during surgical interventions where usually limited observed data, such as a few 2D frames or 1D signals, is available in real-time. We propose a versatile framework for reconstructing 3D motion from such partial data. It discretizes the 3D space into a deformable tetrahedral grid with signed distance values, providing implicit unlimited resolution while maintaining explicit control over motion dynamics. Given an initial 3D model reconstructed from pre-operative full volumetric data, our system, equipped with an universal observation encoder, can reconstruct coherent 3D cardiac motion from full 3D volumes, a few 2D MRI slices or even 1D signals. Extensive experiments on cardiac intervention scenarios demonstrate our ability to generate plausible and anatomically consistent 3D motion reconstructions from various sparse real-time observations, highlighting its potential for multimodal cardiac imaging. Our code and model will be made available at https://github.com/Scalsol/MedTet.

==> bib/figmacro.tex <==
\newif\ifrgb
\rgbfalse

\newif\iffig
\figtrue

\newcommand{\figx}[2]
{
 \iffig
  \includegraphics[width=#1,keepaspectratio]{#2} 
 \else
   \parbox{#1}{#2} 
 \fi
}

\newcommand{\figy}[2]
{
 \iffig
  \includegraphics[height=#1,keepaspectratio]{#2}  
   \else
  \parbox{#1}{#2} 
 \fi
}

\newcommand{\figxy}[3]
{
 \iffig
  \includegraphics[width=#1,height=#2]{#3} 
 \else
   \parbox{#1}{#2}
  \fi
}

\newcommand{\figurecaption}[2]
{
\caption[]{\parbox[t]{#1}{#2}}
}

\newcommand{\fcaption}[1]
{
 \figurecaption{0.9\linewidth}{\small #1}
}

\newcommand{\figdir}[1]
{
\def\figurepath{#1}
}

\renewcommand{\topfraction}{1}
\renewcommand{\dbltopfraction}{1}
\renewcommand{\bottomfraction}{1}
\renewcommand{\textfraction}{.0}
\renewcommand{\floatpagefraction}{1}
\renewcommand{\dblfloatpagefraction}{1}


==> bib/report.tex <==
\usepackage{named}

\usepackage{geometry}
\usepackage{times}
\usepackage{graphics}
\usepackage{graphicx}
\usepackage{subfigure}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{amsthm,amssymb}
\usepackage{color}

\geometry{
 a4paper,
 left=21mm,
 right=21mm,
 top=16mm,
 bottom=16mm,
 }
 
%\setlength{\oddsidemargin}{0.0in}
%\setlength{\topmargin}{-0.125in}
%\setlength{\textwidth}{6.25in}
%\setlength{\textheight}{8.75in}
%\parskip 6pt plus 3pt minus 2pt

\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
\newcommand{\be}{\begin{enumerate}}
\newcommand{\ee}{\end{enumerate}}
\newcommand{\bd}{\begin{description}}
\newcommand{\ed}{\end{description}}
\newcommand{\im}{\item}
\newcommand{\comment}[1]{}
\newcommand{\missing}[1]{\begin{large} {\bf ADD:} {\em #1} \end{large}}
\newcommand{\note}[1]{\begin{center} \noindent\framebox{\begin{minipage}{8cm}{\bf #1}\end{minipage}}\end{center}\\}
\newcommand{\rmk}[1]{{\color{red}{ \bf #1}}}
\newcommand{\red}[1]{{\color{red}{#1}}}
\newcommand{\url}[1]{#1}

\newif\ifsubmit
\submitfalse

\newif\ifdraft
\draftfalse

\newcommand{\dspace}{\renewcommand{\baselinestretch}{1.5}\large\normalsize}
\newcommand{\sspace}{\renewcommand{\baselinestretch}{1.0}\large\normalsize}
\newcommand{\Section}[1]{\section{#1}}
\newcommand{\SubSection}[1]{\subsection{#1}}
\sspace

\renewcommand{\floatpagefraction}{1.0}


==> tabs/supp_tab2.tex <==
\begin{table}[t]
    \centering
    \footnotesize
    \begin{tabular}{lccc}
        \Xhline{1.0pt}
        Method & $CD$ $\downarrow$ & $NC$ $\uparrow$ & $ASSD$ $\downarrow$\\
        \hline
        Voxel (nnU-Net~\cite{isensee2021nnunet}) & 1.644 & 0.5907 & 9.991 \\
        Mesh (Voxel2Mesh*~\cite{Wickramasinghe20}) & 0.7686 & 0.7014 & 10.99 \\
        Implicit (DeepCSR*~\cite{cruz2021deepcsr}) & 0.5698 & 0.7064 & 9.447\\
        \hline
        Ours & \bf 0.5217 & \bf 0.7077 & \bf 9.050 \\ 
        \Xhline{1.0pt}
    \end{tabular}
    \caption{\textit{Quantitative evaluation of static shape reconstruction on the CHAOS dataset.} *: We use the same backbone as ours for a fair comparison. $CD$ and $ASSD$ in $\times 10^{-3}$.}
    \label{tab:static-chaos}
    \vspace{-10px}
\end{table}

==> tabs/supp_tab3.tex <==
\begin{table}[t]
    \footnotesize 
    \centering
    \begin{tabular}{lccc}
        \Xhline{1.0pt}
        Method & $CD$ $\downarrow$ & $NC$ $\uparrow$ & $ASSD$ $\downarrow$\\
        \hline
        Voxel (nnU-Net~\cite{isensee2021nnunet}) & 1.991 & 0.6667 & 1.662 \\
        Mesh (Voxel2Mesh*~\cite{Wickramasinghe20}) & 1.913 & 0.7142 & 1.657 \\
        Implicit (DeepCSR*~\cite{cruz2021deepcsr}) & \bf 1.748 & 0.7379 & \bf 1.647\\
        \hline
        Ours & 1.756 & \bf 0.7594 & 1.659 \\ 
        \Xhline{1.0pt}
    \end{tabular}
    \caption{\textit{Quantitative evaluation of static shape reconstruction on the MMWHS dataset.} *: We use the same backbone as ours for a fair comparison. $CD$ in $\times 10^{-3}$. $ASSD$ in $\times 10^{-2}$.} 
    \label{tab:static-mmwhs}
    \vspace{-10px}
\end{table}

==> tabs/tab_1D.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{c|c}
        \Xhline{1.0pt}
        {Method} & $CD$ \\
        \hline
        Ours & 1.325 \\
        \Xhline{1.0pt}
    \end{tabular}
    \caption{\textit{Quantitative evaluation on 4DM dataset by taking the left myocardium volume as condition.} $CD$ in $\times 10^{-3}$.}
    \label{tab:1d-main}
\end{table}

==> tabs/tab_4dm.tex <==
% already merged. Forgot to keep the orginal 4DM-only table.

\begin{table*}[ht]
    \centering
    \small
    \begin{tabular}{l|c|ccc|ccc}
        \toprule
         \multirow{2}{*}{Method} & \multirow{2}{*}{Category} & \multicolumn{3}{c|}{4DM (Myo)} & \multicolumn{3}{c}{ACDC (3-Average)} \\
&  & 1-Slice & 3-Slice & Full Volume & 1-Slice & 3-Slice & Full Volume \\
        \midrule
        DeepMesh~\cite{Meng23b} & Explicit (Mesh) & - & - & 0.705 & - & - & 1.402  \\
        MeshDeformNet*~\cite{kong2021meshdeform}& Explicit (Mesh) & 1.123 & 0.909 & 0.702 & 2.776 & 2.245 & 1.388 \\
        DeepCSR*~\cite{cruz2021deepcsr} & Implicit (SDF) & 1.179 & 0.922 & 0.733 & 2.887 & 2.336 & 1.422\\
        \midrule
        Ours w/o P3D encoder & Hybrid (Tetrahedra) & 1.337 & 1.203 & 1.053 & 3.294 & 3.023 & 2.866\\
        Ours w/o distillation loss & Hybrid (Tetrahedra) & 1.155 & 0.920 & \bf 0.695 & 2.933 & 2.413 & 1.362\\
        \hline
        Ours & Hybrid (Tetrahedra) & \bf 1.024 & \bf 0.861 & 0.698 & \bf 2.567 & \bf 2.008 & \bf 1.350\\
        \bottomrule
    \end{tabular}
    \vspace{-3mm}
    \caption{\textit{Quantitative evaluation on 4DM and ACDC.} On 4DM, annotations are available for the full training sequences, and metrics on a single class (Myo) are reported. On ACDC, annotations are only available at the ED and ES phases, and 3-structure averages (Myo, LV RV) are reported. *: Our modified version to enable these methods for motion prediction (Sec.~\ref{sec:exp-settings}). $CD$ in $\times 10^{-3}$.}
    \label{tab:4dm-main}
    \label{tab:acdc-main}
\end{table*}

==> tabs/tab_acdc.tex <==
\begin{table*}[ht]
    \centering
    \small
    \begin{tabular}{l|c|ccc}
        \toprule
        Method & Category & 1-Slice & 3-Slice & Full Volume\\
        \midrule
        DeepMesh~\cite{Meng23b} & Explicit (Mesh) & - & - & 1.402 \\
        MeshDeformNet*~\cite{kong2021meshdeform} & Explicit (Mesh) & 2.776 & 2.245 & 1.388 \\
        DeepCSR*~\cite{cruz2021deepcsr} & Implicit (SDF) & 2.887 & 2.336 & 1.422 \\
        \midrule
        Ours w/o P3D encoder & Hybrid (Tetrahedra) & 3.294 & 3.023 & 2.866 \\
        Ours w/o distillation loss & Hybrid (Tetrahedra) & 2.933 & 2.413 & 1.362 \\
        \hline
        Ours & Hybrid (Tetrahedra) & \bf 2.567 & \bf 2.008 & \bf 1.350 \\
        \bottomrule
    \end{tabular}
    \vspace{-3mm}
    \caption{\textit{Quantitative evaluation ACDC, where annotations are only available at the ED and ES phases.} 3-structure (Myo, LV RV) averages are reported. *: Our modified version to enable these methods for motion prediction (Sec.~\ref{sec:exp-settings}). $CD$ in $\times 10^{-3}$. } 
    \label{tab:acdc-main}
\end{table*}
